Nonbacktracking spectral clustering of nonuniform hypergraphs

Spectral methods offer a tractable, global framework for clustering in graphs via eigenvector computations on graph matrices. Hypergraph data, in which entities interact on edges of arbitrary size, poses challenges for matrix representations and therefore for spectral clustering. We study spectral clustering for nonuniform hypergraphs based on the hypergraph nonbacktracking operator. After reviewing the definition of this operator and its basic properties, we prove a theorem of Ihara-Bass type which allows eigenpair computations to take place on a smaller matrix, often enabling faster computation. We then propose an alternating algorithm for inference in a hypergraph stochastic blockmodel via linearized belief-propagation which involves a spectral clustering step again using nonbacktracking operators. We provide proofs related to this algorithm that both formalize and extend several previous results. We pose several conjectures about the limits of spectral methods and detectability in hypergraph stochastic blockmodels in general, supporting these with in-expectation analysis of the eigeinpairs of our studied operators. We perform experiments in real and synthetic data that demonstrate the benefits of hypergraph methods over graph-based ones when interactions of different sizes carry different information about cluster structure.

==> content/algorithms.tex <==
% !TEX root = ../main.tex  

\section{Algorithmic Considerations}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/algorithm-demo.png}
    \caption{
        Illustration of the stages of our clustering algorithm. 
        In this example, we generated a synthetic hypergraph with three clusters of 50 nodes each, with $\ck{2}{} = \ck{3}{} = 6$. 
        95\% of 2-edges and 5\% of 3-edges are within-cluster. 
        (A). 
        First, we compute the spectrum of the approximate matrix $\bJ$, given by \cref{eq:jacobian}. 
        In practice, we compute on the matrix $\bJ'$ described in \Cref{thm:reduced-jacobian}.  
        In this example, there are 8 real eigenvalues outside the bulk, which is demarcated by the circle with radius $\sqrt{\lambda_1}$.  
        (B). 
        Next, we form aggregated eigenvectors of $\bJ$, which we visualize here as matrices. 
        Shown are the signs of the aggregated eigenvectors for the four circled real eigenvalues in (A). 
        The entries are $v_{j;i,s} = \mathrm{sign}\paren*{\sum_{k}\alpha_{ik}^{(s)}}$, with $\valpha$ calculated from $\vu_j$  as in \cref{eq:alpha-beta-def}. 
        Thick horizontal lines separate nodes in different ground-truth clusters. 
        (C). Finally, we cluster the nodes in the space spanned by the columns $\vv_{j;\cdot,s}$ for each aggregate eigenvector $\vv_j$ and cluster $s$.  
        In our example, this space has $8 \times 3 = 24$ dimensions. 
        Here, we visualize the true clusters in two dimension using the t-SNE embedding algorithm~\cite{van2008visualizing}. 
    }
    \label{fig:algorithm}
\end{figure}

















    

\subsection{Fundamental Limitations}

Say some systematic things about the regimes in which the method works here, pose some conjectures re: eigenvalues, that kind of thing. 



\subsection{From Eigenvectors to Clusters}

The operator $\mJ'$ has too many real eigenvalues, and it should have fewer. 
But, it doesn't.  
So, we need to take the corresponding eigenvectors, and figure out how to process them into clusters. 
This is actually a somewhat novel kind of problem, which doesn't arise in the case of graph nonbacktracking because in that case it's unnecessary to explicitly consider $\mJ$ and one can instead consider $\mB$. 

put an illustrative diagram here: hypergraph, matrix, spectrum, PCA


So, how does one get reasonable clusterings out of this? 

k-means, use scree plot for selecting number of clusters, put versions of the triptychs here. 


% \todo{update: nothing wrong with conensus clustering per se, but it loooks like one can also get reasonable clusterings just by doing k-means in an appropriately vectorized version of the eigenvectors}

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{fig/consensus-clustering.png}
%     \caption{(A): 
%         Illustration of consensus clustering in the \texttt{contact-high-school} hypernetwork. 
%         Sign patterns of two aggregated eigenvectors. 
%         Each row corresponds to a node, and each column to one of nine clusters. 
%         (B): 
%         Number of sign agreements for each pair of nodes from the first 100 eigenvectors of the Jacobian $\mJ$. 
%         The maximum number of agreements is $100\times \ell$ = 900. 
%         Nodes are ordered according to a partition produced by the consensus-clustering algorithm with randomized initial condition. 
%         The shown partition has adjusted Rand Index 0.82 against ground-truth labels. 
%     }
%     \label{fig:consensus-clustering}
% \end{figure}














==> content/detectability.tex <==
% !TEX root = main.tex  

\section{Detectability} \label{sec:detectability}

blah blah detectability??
